A Rule for Gradient Estimator Selection, with an Application to Variational Inference

Stochastic gradient descent (SGD) is the workhorse of modern machine learning. Sometimes, there are many different potential gradient estimators that can be used. When so, choosing the one with the best tradeoff between cost and variance is important. This paper analyzes the convergence rates of SGD as a function of time, rather than iterations. This results in a simple rule to select the estimator that leads to the best optimization convergence guarantee. This choice is the same for different variants of SGD, and with different assumptions about the objective (e.g. convexity or smoothness). Inspired by this principle, we propose a technique to automatically select an estimator when a finite pool of estimators is given. Then, we extend to infinite pools of estimators, where each one is indexed by control variate weights. This is enabled by a reduction to a mixed-integer quadratic program. Empirically, automatically choosing an estimator performs comparably to the best estimator chosen with hindsight.

==> sections/ignoreexps.tex <==
% !TEX root = ../main.tex

\section{Experiments and Results}
\label{sec:exps}



This section presents results that empirically validate Alg. \ref{alg:g2tcv} for control variate selection. We tackle inference problems on several probabilistic models using SGVI. We use the plain reparameterization gradient as base estimator and three control variates ($c_1, c_2, c_3$) to reduce its variance.

We use Algorithm \ref{alg:g2tcv} with the set of estimators $\mathcal{G}_\mathrm{Auto}$, that include all estimators that use some (or all, or none) of the available control variates. In this case, selecting an estimator involves selecting what control variates to use and their respective weights.

We compare against using each possible \emph{fixed} subset of control variates with the weights that minimize the estimator's variance. This can be seen as using Algorithm \ref{alg:g2tcv} with the set of estimators $\mathcal{G}_S$, which contains all estimators that use a \emph{fixed} subset of control variates $S\subseteq\{c_1, c_2, c_3\}$. Since all estimators in $\mathcal{G}_S$ use the same control variates, they all have the same cost. Therefore, finding the estimator with optimal cost variance tradeoff (minimum $\hat{G}^2 \hat{T}$) reduces to finding the estimator with minimum variance (which can be done analytically \cite{CVs}). We consider different sets $\mathcal{G}_S$, one for every possible subset of control variates $S\subseteq\{c_1, c_2, c_3\}$.

In short, we compare the results obtained by using Algorithm \ref{alg:g2tcv} with different sets of estimators. The different sets of estimators considered are shown in Table \ref{table:gs}. When used with $\mathcal{G}_\mathrm{Auto}$, Algorithm \ref{alg:g2tcv} selects what control variates to use and their weights. When used with some $\mathcal{G}_S$, the set of control variates is fixed and Algorithm \ref{alg:g2tcv} determine their weights.

\subsection{Experimental details}
\label{sec:exp_details}

\textbf{Tasks and datasets:} We use SGVI on several probabilistic models: (i) Bayesian logistic regression with the datasets Mushrooms and a1a, with a standard normal prior on the weights; (ii) a hierarchical Poisson model with the Frisk dataset \cite{frisk}; and (iii) two variants of a Bayesian neural network with the Red-wine dataset. The difference between the latter two models is on the prior used: a scaled standard normal or a hierarchical distribution. Details for all models are given in the appendix.

\textbf{Variational distribution: } We consider two different variational distributions $q_w(z)$: a Gaussian distribution with a full-rank covariance matrix for the logistic regression models, and a factorized Gaussian distribution (diagonal covariance matrix) for the Bayesian neural networks and the hierarchical Poisson model.

% \textbf{Base gradient estimator: } For the base gradient estimator, $g_\base$, we compute the entropy term $\nabla_w \E_{q_w}[\log q_w(Z)]$ in closed form, and estimate the term $\nabla_w \E_{q_w}[\log p(x, Z)]$ with the reparameterization estimator, $\nabla_w \log p(x,\mathcal{T}_w(\xi))$.\footnote{$\mathcal{T}_w(\xi) = \mu + D^{1/2} \xi$, where $\xi \sim \mathcal{N}(0, I)$, $\mu$ is the mean of $q_w$ and $D^{1/2}$ is the Cholesky factorization of the covariance of $q_w$.}

\textbf{Base gradient estimator: } 
As base gradient estimator, $g_\base$, we use what seems to be the most common estimator. We compute the entropy term \small$\nabla_w \E_{q_w}[\log q_w(Z)]$ \normalsize in closed form, and estimate the term \small$\nabla_w \E_{q_w}[\log p(x, Z)]$ \normalsize with reparameterization.\footnote{Using $\mathcal{T}_w(\xi) = \mu + D^{1/2} \xi$, where $\xi \sim \mathcal{N}(0, I)$, $\mu$ is the mean of $q_w$ and $D^{1/2}$ is the Cholesky factorization of the covariance of $q_w$.}

\textbf{Control variates used: }
\vspace{-0.4cm}
\begin{description} [leftmargin=*] \denselist
  \item[$c_1$:] Difference between the entropy term computed exactly and estimated using reparameterization: \small$c(w, \xi) = \nabla_w \log q_w(\mathcal{T}_w(\xi)) - \nabla_w \E_{q_w} \log q_w(Z)$\normalsize.
  \item[$c_2$:] Control variate by Miller et al. \cite{traylorreducevariance_adam} based on a second order Taylor expansion of $\log p(x, z)$ (Sec \ref{sec:CVSVI}).
  \item[$c_3$:] Difference between the prior term computed exactly and estimated using reparameterization: \small$c(w, \xi) = \nabla_w \log p(\mathcal{T}_w(\xi)) - \nabla_w \E_{q_w} \log p(Z)$\normalsize.
\end{description}

\textbf{Algorithmic details: } We use Algorithm \ref{alg:g2tcv} with different sets of estimators, shown in Table \ref{table:gs}. We use $M = 400$ to estimate $\hat{G}^2$ (except for Logistic regression with the datasets a1a and mushrooms, for which we use $M = 200$). We re-select the optimal estimator three times throughout training, initially, after 10\% of training is done, and after 50\% of training is done.

% In short, when Alg. \ref{alg:g2tcv} is used with the set of estimators $\mathcal{G}_\mathrm{Auto}$, the algorithm selects what control variates to use and their respective weigths. On the other hand, when Alg. \ref{alg:g2tcv} is used with some $\mathcal{G}_S$, the set of control variates used is fixed and the algorithm only determines their weights.

\renewcommand{\arraystretch}{1}
\begin{table}[ht]
  \centering
  \begin{tabular}{llll}
    \hline
    Set of estimators & $c_1$ & $c_2$ & $c_3$\\ \hline
    $\mathcal{G}_1$ & $\m$ & $-$ &$-$ \\
    $\mathcal{G}_2$ & $-$ & $\m$ &$-$ \\
    $\mathcal{G}_3$ &$-$ &$-$ & $\m$ \\
    $\mathcal{G}_{12}$ & $\m$ & $\m$ &$-$ \\
    $\mathcal{G}_{13}$ & $\m$ &$-$ & $\m$ \\
    $\mathcal{G}_{23}$ &$-$ & $\m$ & $\m$ \\
    $\mathcal{G}_{123}$ & $\m$ & $\m$ & $\m$ \\
    $\mathcal{G}_\mathrm{Auto}$ & ? & ? & ? \\
    $\mathcal{G_\mathrm{Base}} = \{g_{\base}\}$ &$-$ &$-$ &$-$ \\ \hline
  \end{tabular}
  \caption{Sets of estimators considered. Each $\mathcal{G}_S$ is identified with the control variates used by estimators $g\in\mathcal{G}_S$. For example, $\mathcal{G}_{12}$ is the set of estimators that use the base estimator and control variates $c_1$ and $c_2$; that is, $\mathcal{G}_{12} = \{g_\mathrm{base} + a_1 c_1 + a_2 c_2 | a_1 \in \mathbb{R}, a_2 \in \mathbb{R}\}$. $\mathcal{G}_\mathrm{Base} = \{g_\mathrm{base}\}$ only contains the base estimator, which does not use any control variates. In the case of $\mathcal{G}_\mathrm{Auto}$, different estimators may use different control variates.}
  \label{table:gs}
\end{table}

\textbf{Optimization details: } We use SGD with momentum ($\beta = 0.9$) and a mini-batch of 5 samples from $q_w(z)$ to form the Monte Carlo gradient estimates. For all models we find an initial set of parameters by optimizing with the base gradient for 300 steps and a fixed learning rate of $10^{-5}$.

% \tg{Add the Adam initialization step. I'll try to fix this. In any case, what do you think would be the least hurting way we can put this? Or do you think this is unacceptable and must be fixed? We could initialize to the MAP? Other options for initialization?}

% \renewcommand{\arraystretch}{1}
% \begin{table*}[t]
%   \centering
%   \begin{tabular}{cccccccccc}
%     \hline
%     Control Variate & $\mathcal{G}_1$ & $\mathcal{G}_2$ & $\mathcal{G}_3$ & $\mathcal{G}_{12}$ & $\mathcal{G}_{13}$ & $\mathcal{G}_{23}$ & $\mathcal{G}_{123}$ & $\mathcal{G}_\mathrm{Auto}$ & $\mathcal{G_\mathrm{Base}} = \{g_{\base}\}$ \\ \hline
%     $c_1$ & $\m$     & $-$     & $-$      & $\m$      & $\m$      & $-$       & $\m$      & $?$ & $-$\\
%     $c_2$ & $-$      & $\m$    & $-$      & $\m$      & $-$       & $\m$      & $\m$      & $?$ & $-$ \\
%     $c_3$ & $-$      & $-$     & $\m$     & $-$       & $\m$      & $\m$      & $\m$      & $?$ & $-$ \\ \hline
%   \end{tabular}
%   \caption{Each $\mathcal{G}_S$ is identified with a subscript that indicates what control variates are used by estimators $g\in\mathcal{G}_S$. $\mathcal{G}_\mathrm{Base}$ only contains the base estimator, which does not use any control variates. In the case of the full set $\mathcal{G}_\mathrm{Auto}$, different estimators may use different control variates.}
%   \label{table:gs}
% \end{table*}

\subsection{Results}

\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.31\linewidth]{./figures/exps_bnnrw.pdf}
  \includegraphics[width=0.31\linewidth]{./figures/exps_bnnrw2.pdf}
  \includegraphics[width=0.31\linewidth]{./figures/exps_friskm.pdf}

  \includegraphics[width=0.31\linewidth]{./figures/exps_logistic-mushrooms.pdf}
  \includegraphics[width=0.31\linewidth]{./figures/exps_logistic-a1a.pdf}
  % \includegraphics[width=0.31\linewidth]{./figures/exps_logistic-australian.pdf}

  % \includegraphics[width=0.31\linewidth]{./figures/exps_logistic-splice.pdf}
  % \includegraphics[width=0.31\linewidth]{./figures/exps_logistic-ionosphere.pdf}
  % \includegraphics[width=0.31\linewidth]{./figures/exps_logistic-sonar.pdf}
  \caption{\textbf{Automatically selecting what control variates to use performs comparably to the best fixed set of control variates chosen with hindsight.} ``ELBO vs Time'' plots obtained using Alg. \ref{alg:g2tcv} to select what control variates to use and their weights (Alg. \ref{alg:g2tcv} with $\mathcal{G}_\mathrm{Auto}$, plotted in black). We compare against using different fixed subsets of control variates with the weights that minimize the estimator's variance. Six different models were considered: two variants of a Bayesian neural network, a hierarchical Poisson model, and Bayesian logistic regression with three datasets. Lines are identified as follows: ``Auto'' stands for using Alg. \ref{alg:g2tcv} to select what control variates to use and their weights, ``Base'' stands for optimizing using the base gradient alone, ``12'' stands for using the fixed set of control variates $\{c_1, c_2\}$ with the minimum variance weights, ``13'' stands for using the fixed set of control variates $\{c_1, c_3\}$, and so on.}
  \label{fig:elbotime3}
\end{figure*}

Simulations were performed for several different learning rates, and the one that led to the best results was chosen. Results shown are the average over 20 runs. Fig. \ref{fig:elbotime3} shows the optimization results (``ELBO vs. Time'' plots). It can be observed that automatically selecting what control variates to use and their weights (using Alg. 2 with $\mathcal{G}_\mathrm{Auto}$) leads to good results, as good as the ones obtained using the best fixed set of control variates chosen retrospectively. It can also be observed that results depend heavily on the model considered. For instance, for some models using the base gradient without any control variates appears to be the best choice (logistic regression (a1a) and BNN-B), while for others it is suboptimal (BNN-A).

Fig. \ref{fig:final} shows a summary of the results to ease comparison. For each model, it shows the final training ELBO achieved by using each possible fixed subset of control variates and the automatically chosen ones. It can be observed that there is no fixed subset of control variates that performs well accross all models. However, using the automatically chosen control variates does.

% that allows an easy comparison between using different fixed subsets of control variates and the automatically chosen ones.
% For each model the ELBO values are scaled between 0 and 1 (where the lowest ELBO correspond to 0 and the highest to 1).
% y-axis is scaled for each model to ease comparison and visualization.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\linewidth]{./figures/final.pdf}
  \caption{\textbf{The automatically chosen control variates perform well in all models.} Final training ELBO obtained by using each subset of control variates and the automatically chosen ones. Y-axis is scaled (between 0 and 1) for each model.}
  \label{fig:final}
\end{figure}

It is clear from Fig. \ref{fig:elbotime3} that Alg. \ref{alg:g2tcv} ran with $\mathcal{G}_\mathrm{Auto}$ selects a ``good'' set of control variates (and weights). What control variates are being chosen? This is shown in Table \ref{table:choices}. It can be observed that the algorithm makes different choices for different models, and that the control variates chosen depend on the stage of the training process (initially, or later stages). As shown in Fig. \ref{fig:elbotime3}, these choices lead to good results.

\renewcommand{\arraystretch}{1.1}
\begin{table}[ht]
\begin{small}
  \centering
  \begin{tabular}{llll}
    \hline
    \multirow{2}{*}{Model} & \multicolumn{3}{c}{Time of choice} \\ \cline{2-4}
    & $T = 0$ & $T = T_{opt}/10$ & $T = T_{opt}/2$\\ \hline
    % Log Reg (aus) & $\{c_2\}$ & $\{c_1\}$ & $\{c_1\}$ \\
    Log Reg (a1a) & $\{c_1, c_3\}$ & $\{c_1\}$ & $\{c_1\}$ \\
    Log Reg (mush) & $-$ & $-$ & $\{c_1\}$ \\
    Hier Poisson & $\{c_2\}$ & $\{c_2\}$ & $\{c_2\}$ \\
    BNN-A & $\{c_3\}$ & $\{c_1\}$ & $\{c_1\}$ \\
    BNN-B & $-$ & $-$ & $-$ \\ \hline
  \end{tabular}
  \caption{\textbf{Algorithm \ref{alg:g2tcv} selects different control variates for different models.} The table shows the control variates chosen by Algorithm \ref{alg:g2tcv} when ran with the set of estimators $\mathcal{G}_\mathrm{Auto}$, at three different selection times. $\{c_i\}$ means that the algorithm selected control variate $c_i$ (and discarded the other ones), $\{c_i, c_j\}$ that the algorithm selected control variates $c_i$ and $c_j$ (discarded the other one), and $-$ that no control variates are used (optimization is performed using the base gradient alone. All control variates were discarded). %(Simulations are performed several times. For a same model, different choices may be made in different runs. The table shows the ``most popular'' choice across all runs.)
  }
  \label{table:choices}
\end{small}
\end{table}

% \tg{Say sth about choices not being always the same, and that even if using the same c all the time is not good, it may be good at some points during optimization.}

% We also show ``Final ELBO vs $\hat{G}^2\hat{T}$'' plots in Fig. \ref{fig:elbog2t}. For each set of estimators $\mathcal{G}$ used with Algorithm \ref{alg:g2tcv} we plot the final ELBO after training against the average $\hat{G}^2 \hat{T}$ value of the estimator used. It can be observed that, in general, the use of estimators with lower $\hat{G}^2 \hat{T}$ tends to lead to better ELBOs. In particular, when used with $\mathcal{G}_\mathrm{Auto}$, Algorithm \ref{alg:g2tcv} selects estimators that are among the ones with lower $\hat{G}^2 \hat{T}$, which leads to high ELBOs.

% \begin{figure*}[ht]
%   \centering
%   \includegraphics[width=0.31\linewidth]{./figures/ELBOG2T_bnnrw.pdf}
%   \includegraphics[width=0.31\linewidth]{./figures/ELBOG2T_bnnrw2.pdf}
%   \includegraphics[width=0.31\linewidth]{./figures/ELBOG2T_friskm.pdf}

%   \includegraphics[width=0.31\linewidth]{./figures/ELBOG2T_logistic-mushrooms.pdf}
%   \includegraphics[width=0.31\linewidth]{./figures/ELBOG2T_logistic-a1a.pdf}
%   \includegraphics[width=0.31\linewidth]{./figures/ELBOG2T_logistic-australian.pdf}
%   \caption{Final ELBO after training vs. average $\hat{G}^2 \hat{T}$ values throughout optimization for different models. Each point in the plots is identified following the convention from Fig. \ref{fig:elbotime3}. }
%   \label{fig:elbog2t}
% \end{figure*}

% \textbf{Automatically picking an estimator to minimize $\mathbf{G^2 T}$ performs similarly to minimizing $\mathbf{G^2}$ with the best set of control variates chosen in hindsight.} }

% \renewcommand{\arraystretch}{1}
% \begin{table*}[t]
% \begin{small}
%   \centering
%   \begin{tabular}{llllllllll}
%     \hline
%     Model & $\{g_{\base}\}$ & $\mathcal{G}_1$ & $\mathcal{G}_2$ & $\mathcal{G}_3$ & $\mathcal{G}_{12}$ & $\mathcal{G}_{13}$ & $\mathcal{G}_{23}$ & $\mathcal{G}_{123}$ & $\mathcal{G}_\mathrm{Auto}$ \\ \hline
%     Bayesian NN - A & -159.23 & -154.21 & -155.91 & -154.40 & -155.56 & -154.51 & -155.39 & -155.28 & -154.33\\ 
%     Bayesian NN - B & -479.37 & -486.53 & -502.50 & -487.11 & -501.35 & -490.86 & -499.83 & -498.38 & -479.82\\ 
%     Log. regr. (mushrooms) & -209.59 & -191.41 & -543.72 & -191.24 & -374.19 & -201.40 & -356.98 & -375.97 & -187.78\\ 
%     Log. regr. (sonar) & -110.20 & -110.05 & -110.07 & -110.37 & -110.07 & -110.08 & -110.08 & -110.07 & -110.04\\ \hline
%   \end{tabular}
%   \vspace{0.15cm}
%   \caption{Final ELBO after training using Alg.}
%   \label{table:gs}
% \end{small}
% \end{table*}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.3\linewidth]{./figures/ELBO-time-new-labelmushrooms.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/ELBO-time-new-labela1a.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/ELBO-time-new-labela8a.pdf}

%   \includegraphics[width=0.3\linewidth]{./figures/ELBO-time-new-labelsplice.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/ELBO-time-new-labelionosphere.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/ELBO-time-new-labelsonar.pdf}
%   \caption{\textbf{Automatically picking an estimator to minimize $\mathbf{G^2 T}$ performs similarly to minimizing $\mathbf{G^2}$ with the best set of control variates chosen in hindsight.} ELBO vs Time plots obtained when using estimators automatically chosen from $\mathcal{G}$ and each $\mathcal{G}_S$, for six different datasets. Each line's label contains the control variates considered. "Auto" chooses what control variates to include using a MIQCP. This is compared to fixing the included control variates and simply minimizing $G^2$. Overheads incurred by the estimators (estimating $G^2$, profiling, MIQCP) are included in the time.}
%   \label{fig:elbotime3}
% \end{figure}

% Fig. \ref{fig:felbog2t} shows the ELBO after optimization vs. empirical $G^2 T$ values for the automatically chosen estimators from $\mathcal{G}$ and each $\mathcal{G}_S$. Results show that optimizing using estimators with lower $G^2 T$ result in higher ELBOs, validating the $G^2 T$ principle. Results also show that "Auto" selects estimators with lowest empirical $G^2 T$, which lead to highest ELBO, validating the estimator selection algorithm.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.3\linewidth]{./figures/FE-G2T-mushrooms.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/FE-G2T-a1a.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/FE-G2T-a8a.pdf}

%   \includegraphics[width=0.3\linewidth]{./figures/FE-G2T-splice.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/FE-G2T-ionosphere.pdf}
%   \includegraphics[width=0.3\linewidth]{./figures/FE-G2T-sonar.pdf}
%   \caption{\textbf{The use of estimators with lower $\mathbf{G^2T}$ tend to lead to better (higher) ELBOs. "Auto" is near the best performance in all cases.} ELBO after training vs. G2T for estimators automatically chosen from $\mathcal{G}$ and each $\mathcal{G}_S$, for different datasets.}
%   \label{fig:felbog2t}
% \end{figure}


